ECH0EZ: Estimating the Hubble constant with ZTF SN Ia DR2

Type Ia supernovae (SNe Ia) are instrumental for a precise measurement of the Hubble constant ($H_0$) from the local distance ladder, yet the data used hitherto for this purpose are inhomogeneous and subject to severe selection effects. We present the first, preliminary, cosmological analysis of 772 SNe Ia from the Zwicky Transient Facility's second data release: an untargeted single-telescope sample whose volume-limited subset (z<0.06) is largely free of Malmquist bias. We correct the public data for known instrumental and calibration biases and the redshifts for peculiar motions. Using the 42 SH0ES calibrators (their host distances computed from Cepheids and geometric anchors) and a Bayesian hierarchical model of SN Ia standardisation, dust extinction, redshift and calibration uncertainties, we infer $H_0 = (71.6 \pm 1.5)$ km/s/Mpc after marginalising over deceleration with a flat prior (or $(72.3 \pm 1.1)$ km/s/Mpc if a prior on matter density from Pantheon+ is imposed), with the uncertainty dominated by the number of calibrators. We demonstrate robustness to the choice of light-curve and Milky Way dust models and to extensions of the model to include peculiar-velocity correlations, a host-mass step, and two stretch populations. These results are in agreement with previous distance-ladder measurements and $2.7\sigma$ ($4.1\sigma$) away from the value obtained from Planck data, suggesting that the resolution of the Hubble tension lies outside of SNe Ia---or the distance ladder entirely.

==> lib/extra/inference/shortcuts.tex <==
\newoperator{\altprob}{\tilde{p}}

\shortcut{\aparams}{\variable{\psi}}
\shortcut{\iparams}{\variable{\theta}}
\shortcut{\nparams}{\variable{\nu}}
\shortcut{\gparams}{\variable{\gamma}}
\shortcut{\lparams}{\variable{\lambda}}

\shortcut{\data}{\variable{d}}
\newcommand{\targetlabel}{\mathrm{o}}
\newcommand{\target}[2][\targetlabel]{#2_{#1}}
\newcommand{\tdata}[1][\targetlabel]{\target{\data}}
\shortcut{\dataset}{\variable{D}}
\newcommand{\tdataset}[1][\targetlabel]{\target{\dataset}}
\shortcut{\metadata}{\variable{a}}


\newcommand{\fidindex}[1]{#1_{\mathrm{fid}}}
\newcommand{\fidiparams}{\fidindex{\iparams}}
\newcommand{\fidgparams}{\fidindex{\gparams}}

\shortcut{\nobj}{N_{\mathrm{obj}}}
\newmathcommand{\objindexlabel}{i}
\newcommand{\objindex}[2][\objindexlabel]{#2^{#1}}
\newcommand{\objdata}{\objindex{\data}}
\newmathcommand{\objlparams}{\smash{\objindex{\lparams}}\vphantom{\objdata}}
\newcommand{\objmetadata}{\objindex{\metadata}}

\newcommand{\objdataset}[1][\objindexlabel]{\ensuremath{\set{\objindex[#1]{\data}}}\xspace}
\newcommand{\tobjdataset}[1][\objindexlabel]{\ensuremath{\set{\dosmash{\objindex[#1]{\tdata}}\vphantom{\objindex[#1]{\data}}}}\xspace}


% selection
\shortcut{\ntot}{N_{\textrm{tot}}}
\shortcut{\nsel}{N_{\textrm{sel}}}
\shortcut{\exptot}{\expval{\ntot}}

\newcommand{\seloidx}{\objindexlabel}
\newmathcommand{\selmidx}{j}

\shortcut{\selind}{S}
\newcommand{\seloind}[1][\seloidx]{\ensuremath{\mathfrak{s}\ifblank{#1}{}{^{#1}}}\xspace}
\newcommand{\selmind}[1][\selmidx]{\ensuremath{\mathfrak{m}\ifblank{#1}{}{^{#1}}}\xspace}

\newcommand{\seloobjind}{\objindex[\seloidx]{\selind}}
\newcommand{\selmobjind}{\objindex[\selmidx]{\selind}}
\newcommand{\selodata}{\objindex[\seloidx]{\data}}
\newcommand{\selmdata}{\objindex[\selmidx]{\data}}
\newmathcommand{\selolparams}{\dosmash{\objindex[\seloidx]{\lparams}}\vphantom{\selodata}}
\newcommand{\selmlparams}{\dosmash{\objindex[\selmidx]{\lparams}}\vphantom{\selmdata}}


\newmathcommand{\odataset}{\set{\selodata}}
\newmathcommand{\mdataset}{\set{\selmdata}}
\newmathcommand{\oindset}{\set{\seloind}}
\newmathcommand{\mindset}{\set{\selmind}}


\newmathcommand{\igindexlabel}{g}
\newcommand{\igindex}[2][\igindexlabel]{#2_{#1}}
\newcommand{\igiparams}{\igindex{\iparams}}

\shortcut{\iggparams}{\dosmash{\igindex{\gparams}}\vphantom{\gparams}}
\shortcut{\iglparams}{\dosmash{\igindex{\lparams}}\vphantom{\lparams}}
\shortcut{\igobjlparams}{\dosmash{\objindex{\igindex{\lparams}}}\vphantom{\objlparams}}

\NewDocumentCommand{\prior}{O{\iparams}}{\ensuremath{\prob(#1)}\xspace}
\NewDocumentCommand{\evidence}{G{\data}}{\ensuremath{\prob(#1)}\xspace}
\NewDocumentCommand{\joint}{O{\iparams} G{\data}}{\ensuremath{\prob({#1},{#2})}\xspace}
\NewDocumentCommand{\posterior}{O{\iparams} G{\data}}{\ensuremath{\prob({#1} \given {#2})}\xspace}
\NewDocumentCommand{\likelihood}{O{\iparams} G{\data}}{\ensuremath{\prob({#2} \given {#1})}\xspace}

\newoperator[]{\pgrad}{\grad}

\NewDocumentCommand{\likefn}{O{\iparams} G{\tdata}}{\ensuremath{\opbraces{L_{#2}}(#1)}\xspace}
\NewDocumentCommand{\thescore}{O{\iparams} G{\data}}{\ensuremath{\pgrad[#1]\ln\likelihood[#1]{#2}}\xspace}

\newoperator{\estprob}{q}
\NewDocumentCommand{\estpost}{O{\iparams} G{\data}}{\ensuremath{\estprob(#1 \given #2)}\xspace}
\NewDocumentCommand{\estlike}{O{\iparams} G{\data}}{\ensuremath{\estprob(#2 \given #1)}\xspace}

\newcustomabbreviation[first={Kullback\Endash Leibler (KL) divergence}]{kl}{KL divergence}{Kullback\Endash Leibler divergence}
\newcommand{\KL}[3][\,\Vert\,]{\ensuremath{\opbraces{\operatorname{KL}}[#2 #1 #3]}\xspace}
\newcustomabbreviation[first={Jensen\Endash Shannon (JS) divergence}]{js}{JS divergence}{Jensen\Endash Shannon divergence}
\newmathcommand{\JS}[2]{\opbraces{\operatorname{JS}}[#1,#2]}
\newmathcommand{\ELBO}[2]{\ELBO*[#1 \,\Vert\, #2]}
\WithSuffix\newcommand\ELBO*{\opbraces{\operatorname{ELBO}}}

% NRE
\shortcut{\Loss}{\mathcal{L}}
\shortcut{\nnparams}{\variable{\Phi}}

\newoperator{\nreratio}{r}
\shortcut{\nreapprox}{\hat{\nreratio}}

\newcommand{\nncomp}[1]{\ifmmode\mathtt{#1}\else\texttt{#1}\fi}
\newoperator[\nncomp]{\Summariser}{Summariser}
\newoperator[\nncomp]{\ParamHead}{ParamHead}
\newoperator[\nncomp]{\SummaryHead}{SummaryHead}
\newoperator[\nncomp]{\RatioEstimator}{RatioEstimator}


\newcommand{\nnvar}[1]{\pmb{\mathtt{#1}}}
\shortcut{\nndata}{\nnvar{d}}
\shortcut{\nnmeta}{\nnvar{a}}
\shortcut{\nngparams}{\nnvar{\gamma}_{\igindexlabel}}
\shortcut{\nnlparams}{\nnvar{\lambda}_{\igindexlabel}}
\shortcut{\nnsummary}{\nnvar{S}}
\newcommand{\nnlsummary}{\nnsummary_{\iglparams}}

% Truncation
\shortcut{\trunc}{T}
\newcommand{\truncprob}[1][\tdata]{\altprob[\trunc(#1)]}
\NewDocumentCommand{\truncprior}{O{\iparams} G{\tdata}}{\ensuremath{\truncprob[#2](#1)}\xspace}

% QQ

\newabbreviation{pdf}{PDF}{probability density function}
\newabbreviation{cdf}{CDF}{cumulative distribution function}
\newcustomabbreviation[first={probability\Endash probability (P\Endash P) plot}]{ppplot}{P\Endash P plot}{probability\Endash probability plot}

\newcommand{\bcumulative}{\cumulative[\mathrm{B}]}
\newcommand{\fcumulative}{\cumulative[\mathrm{f}]}

\newcommand{\testlabel}{\mathrm{t}}
\newcommand{\test}[2][\testlabel]{#2_{#1}}
\newcommand{\testdata}{\test{\data}}
\newcommand{\testiparams}{\test{\iparams}}
\newmathcommand{\testjoint}{\altjoint[\testiparams]{\testdata}}

\shortcut{\region}{\Gamma}
\shortcut{\confregion}{C}

\shortcut{\cred}{\gamma}
\newcommand{\altcred}{\cred^{*}}
\newcommand{\credfn}[1][\estprob]{\cred_{#1}}
\newcommand{\invcredfn}[1][\estprob]{\credfn[#1]^{-1}}

\shortcut{\conf}{\digamma}
\newcommand{\fixediparams}{\test[*]{\iparams}}
\shortcut{\reqcred}{\hat{\cred}}
%\shortcut{\fullreqquantile}{\opbraces{\reqquantile}(\iparamsnull, \altquantile)}

% Model selection
\shortcut{\Model}{\mathcal{M}}
\shortcut{\aModel}{M}
\shortcut{\nmods}{N_{\mathrm{mod}}}
\newmathcommand{\modidxlabel}{m}
\newcommand{\modidx}[2][\modidxlabel]{#2_{#1}}
\newcommand{\mModel}[1][\modidxlabel]{\modidx[#1]{\aModel}}
\newcommand{\maparams}[1][\modidxlabel]{\modidx[#1]{\aparams}}

\newoperator{\Refinedness}{Refinedness}
\newoperator{\Reliability}{Reliability}



\newabbreviation{dag}{DAG}{directed acyclic graph}
\newabbreviation{hl}{HL}{highest-likelihood}
\newabbreviation{hpd}{HPD}{highest posterior density}
\newabbreviation{drp}{DRP}{distance to random point}

\newabbreviation{imnn}{IMNN}{information-maximising neural network}
\newabbreviation{vmim}{VMIM}{variational mutual-information maximisation}


==> lib/extra/inference/style.tex <==
\pgfplotsset{
	PP plot/.style={
		no markers, legend pos=north west, legend style={draw=none},
		xmin=0, xmax=1, ymin=0, ymax=1, enlargelimits=0.05,
		xlabel={nominal credibility}, ylabel={empirical coverage},
		xticklabel={\pgfmathparse{\tick*100}\SI[round-mode=places,round-precision=0]{\pgfmathresult}{\percent}},
		yticklabel={\pgfmathparse{\tick*100}\SI[round-mode=places,round-precision=0]{\pgfmathresult}{\percent}},
		background shade/.style={
			forget plot, surf, shader=interp, colormap name=midtraffic, point meta=explicit,
			opacity=0.3
		},
		diag/.style={
			forget plot, Greys-H, ultra thin, dashed,
			every node/.append style={anchor=base, sloped, pos=0.75},
			undercovering node/.style={yshift=-1.2em, node contents={undercovering}},
			conservative node/.style={yshift=0.8em, node contents={conservative}},
		},
		execute at begin axis={
%			\addplot[background shade, mesh/cols=2, mesh/rows=2] coordinates {
%				(0, 0) [0]  (1, 0) [1]
%				(0, 1) [-1]  (1, 1) [0]
%			};
			\addplot[diag] coordinates {(0, 0) (1, 1)} node [undercovering node] {} node [conservative node] {};
		}
	},
	Bayesian PP plot/.style={PP plot, ylabel={Bayesian empirical coverage},}
}


==> lib/extra/sn/glossary.tex <==
\edef\aenoxspace{\ae}
\appto{\ae}{\xspace}
\newcommand{\Ianoxspace}{\Rnum{1}a}
\newcommand{\Ia}{\Ianoxspace\xspace}

% noxspace is needed if you'll use a macro inside a siunitx unit....
\newcommand{\SN}{SN\xspace}
\newcommand{\SNae}{SN\aenoxspace\xspace}
\newcommand{\SNIa}{SN~\Ianoxspace\xspace}
\newcommand{\SNaeIa}{SN\aenoxspace~\Ianoxspace\xspace}

\newabbreviation[shortplural={\SNae}, longplural={supernov\ae}]{sn}{\SN}{supernova}
\newabbreviation[shortplural={\SNaeIa}, longplural={type~\Ia supernov\ae}]{snia}{\SNIa}{type~\Ia supernova}
\newabbreviation[shortplural={CC \SNae}, longplural={core-collapse supernov\ae}]{ccsn}{CC \SN}{core-collapse supernova}
\newabbreviation[shortplural={SL\SNae}, longplural={superluminous supernov\ae}]{slsn}{SL\SN}{superluminous supernova}

\newabbreviation{sd}{SD}{single-degenerate}
\newabbreviation{dd}{DD}{double-degenerate}
\newabbreviation{dtd}{DTD}{delay-time distribution}
\newabbreviation{dlr}{DLR}{directional light radius}


%SURVEYS
\newcommand{\ASASSN}{ASAS-\SN}
\newabbreviation[category=wordacro]{asassn}{\ASASSN}{{\scshape A}ll {\scshape S}ky {\scshape A}utomated {\scshape S}urvey for {\scshape S}uper{\scshape n}ov\aenoxspace}
\newabbreviation{psst}{PSST}{\acrshort{psst} Survey for Transients}
\newcommand{\Pantheon}{Pantheon\xspace}
\newcommand{\PantheonPlus}{Pantheon+\xspace}
\newcommand{\SHoES}{S\Ho{}ES\xspace}
\newabbreviation[category=wordacro]{sh0es}{\SHoES}{{\scshape S}upernovae and \Ho for the {\scshape e}quation of {\scshape s}tate of dark energy}
\newabbreviation{cfa}{CfA}{Harvard-Smithsonian Center for Astrophysics}
\newabbreviation{bsnip}{B\SN{}\Rnum{1}P}{Berkeley \SNIa Program}
\newabbreviation[category=wordacro]{loss}{Loss}{{\scshape L}ick {\scshape O}bservatory {\scshape s}upernova {\scshape s}earch}
\newabbreviation[category=wordacro]{essence}{Essence}{{\scshape E}quation of {\scshape s}tate: {\scshape s}up{\scshape e}r{\scshape n}ov\ae trace {\scshape c}osmic {\scshape e}xpansion}
\newabbreviation{snls}{SNLS}{SuperNova Legacy Survey}
\newabbreviation{csp}{CSP}{Carnegie Supernova Project}
\newcommand{\Foundation}{Foundation\xspace}
\newcommand{\SweetSpot}{SweetSpot\xspace}
\newsavebox{\dehvilssavebox}
\newabbreviation[category=wordacro]{dehvils}{Deh\textsubscript{0}\!vils}{{\scshape D}ark {\scshape e}nergy, \Ho, and peculiar {\scshape v}elocities using {\scshape i}nfrared {\scshape l}ight from {\scshape s}upernov\ae}

\newabbreviation[category=wordacro]{raisin}{Raisin}{\SNIa in the \acrshort{ir}}
\newabbreviation{jla}{JLA}{joint light-curve analysis}

% MODELS
\newignoredglossary{snmodel}
\setabbreviationstyle[snmodel]{short-long}
\setabbreviationstyle[wordsnmodel]{short-sc-long}

\newcommand{\snmodelling}[1]{\acrshort*{#1}\xspace}
\newcommand{\newsnmodel}[3][]{\newcommand#2{\snmodelling{#3}}}


\newabbreviation[category=snmodel, type=snmodel]{mlcs}{MLCS}{Multicolor Light-Curve Shape}
    \newsnmodel{\MLCS}{mlcs}
\newabbreviation[category=wordsnmodel, type=snmodel]{salt}{salt}{{\scshape s}pectral {\scshape a}daptive {\scshape l}ight-curve {\scshape t}emplate}
    \newsnmodel{\SALT}{salt}
\newabbreviation[category=wordsnmodel, type=snmodel]{snemo}{snemo}{{\scshape s}uper{\scshape n}ova {\scshape em}pirical {\scshape m}odels}
    \newsnmodel{\SNEMO}{snemo}
    \newcommand{\hyperSNEMO}{\hypercite{Sanders_2018}{\SNEMO}\xspace}
\newabbreviation[category=wordsnmodel, type=snmodel]{sugar}{sugar}{{\scshape su}pernova {\scshape g}enerator {\scshape a}nd {\scshape r}econstructor}
    \newsnmodel{\SUGAR}{sugar}
    \newcommand{\hyperSUGAR}{\hypercite{Leget_2020}{\SUGAR}\xspace}
\defineverb{\SNooPy}{SN(oo)Py}
\newcommand{\suPAErnova}{{\scshape suPAErnova}\xspace}
\newabbreviation[category=wordsnmodel, type=ignore, type=snmodel]{Bahamas}{Bahamas}{{\scshape Ba}yesian {\scshape h}ier{\scshape a}rchical {\scshape m}odeling for the {\scshape a}nalysis of {\scshape s}upernova cosmology}
    \newsnmodel{\BAHAMAS}{Bahamas}

\newcommand{\BayeSN}{BayeSN\xspace}
    \newcommand{\hyperBayeSN}{\hypercite{Mandel_2022}{\BayeSN}\xspace}
\newcommand{\SimpleBayeSN}{Simple-\BayeSN}
    \newcommand{\hyperSimpleBayeSN}{\hypercite{Mandel_2017}{\SimpleBayeSN}\xspace}
\newabbreviation[category=wordsnmodel, type=snmodel]{bird-snack}{bird-snack}{{\scshape B}ayesian {\scshape i}nference of dust law $R_V$ {\scshape d}istributions using {\scshape sn}~\Ia{} {\scshape a}pparent {\scshape c}olours at pea{\scshape k}}
    \newsnmodel{\BIRDSNACK}{bird-snack}
    \newcommand{\hyperBIRDSNACK}{\hypercite{Ward_2023}{\BIRDSNACK}\xspace}
\newabbreviation[category=wordsnmodel, type=snmodel]{unity}{unity}{{\scshape u}nified {\scshape n}onlinear {\scshape i}nference for {\scshape t}ype-\Ia cosmolog{\scshape y}}
    \newsnmodel{\UNITY}{unity}
    \newcommand{\hyperUNITY}{\hypercite{Rubin_2023}{\UNITY}\xspace}
\newcommand{\Steve}{Steve\xspace}
    \newcommand{\hyperSteve}{\hypercite{Hinton_2019}{\Steve}\xspace}
\newabbreviation[category=wordsnmodel, type=snmodel]{abyss}{abyss+}{{\scshape a}pplication of {\scshape B}a{\scshape y}esian graphs to \SNIa data analy{\scshape s}i{\scshape s} and compre{\scshape ss}ion}
    \newsnmodel{\ABYSS}{abyss}
\newabbreviation[category=wordsnmodel, type=snmodel]{beams}{beams}{{\scshape B}ayesian {\scshape e}stimation {\scshape a}pplied to {\scshape m}ultiple {\scshape s}pecies}
    \newsnmodel{\BEAMS}{beams}
    \newcommand{\hyperBEAMS}{\hypercite{Kunz_2007}{\BEAMS}\xspace}
\newcommand{\zBEAMS}{$\z$\BEAMS}
    \newcommand{\hyperzBEAMS}{\hypercite{zBEAMS}{\zBEAMS}\xspace}
\newabbreviation[category=snmodel, type=snmodel]{bbc}{BBC}{\BEAMS with bias correction}
    \newsnmodel{\BBC}{bbc}
    \newcommand{\hyperBBC}{\hypercite{BBC}{\BBC}\xspace}

\newcommand{\PhotozSNthesis}{Photo-\z{}\SN{}thesis\xspace}
    \newcommand{\hyperPhotozSNthesis}{\hypercite{Qu_2023a}{\PhotozSNthesis}\xspace}


\defineverb{\SNANA}{SNANA}
\defineverb{\sncosmo}{sncosmo}
\defineverb{\skysurvey}{skysurvey}
\defineverb{\slicsim}{slicsim}
\newabbreviation[type=software]{slicsim}{SLiCsim}{{\scshape s}upernova {\scshape li}ght-{\scshape c}urve {\scshape s}imulator}

\newabbreviation{spcc}{SPCC}{supernova photometric classification challenge}
\newabbreviation[category=wordacro]{plasticc}{plasticc}{{\scshape p}hotometric \acrshort*{lsst} {\scshape as}tronomical {\scshape ti}me-series {\scshape c}lassification {\scshape c}hallenge}
    \newsnmodel{\plasticc}{plasticc}
    \newcommand{\hyperplasticc}{\hypercite{Kessler_2019}{\plasticc}\xspace}
\newabbreviation[category=wordacro]{elasticc}{elasticc}{{\scshape e}xtended \acrshort*{lsst} {\scshape as}tronomical {\scshape ti}me-series {\scshape c}lassification {\scshape c}hallenge}
    \newsnmodel{\elasticc}{elasticc}

\defineverb{\avocado}{avocado}
    \newcommand{\hyperavocado}{\hypercite{Boone_2019}{\avocado}\xspace}
\newabbreviation[category=wordsnmodel,type=snmodel]{staccato}{staccato}{{\scshape s}yn{\scshape th}etically {\scshape a}ugmented light-{\scshape c}urve {\scshape c}lassific{\scshape at}i{\scshape o}n}
    \newsnmodel{\staccato}{staccato}
    \newcommand{\hyperstaccato}{\hypercite{Revsbech_2018}{\staccato}\xspace}
\newcommand{\SuperNNova}{SuperNNova\xspace}
\newcommand{\SupeRAENN}{SuperNNova\xspace}
\newabbreviation[category=wordsnmodel,type=snmodel]{scone}{scone}{{\scshape s}upernova {\scshape c}lassification with a {\scshape co}nvolutional {\scshape ne}ural {\scshape ne}twork}
    \newsnmodel{\SCONE}{scone}

\defineverb{\Prospector}{Prospector}
\newcommand{\Prospectora}{\Prospector{\Hyphdash*}α\xspace}
\newcommand{\Prospectorb}{\Prospector{\Hyphdash*}β\xspace}

\defineverb{\Speculator}{Speculator}
\newcommand{\Speculatora}{\Speculator{\Hyphdash*}α\xspace}
    \newcommand{\hyperSpeculator}{\hypercite{Alsing_2020}{\Speculator}\xspace}

==> lib/extra/sn/shortcuts.tex <==
\shortcut{\nsn}{N_{\textrm{SN}}}
\shortcut{\nobs}{N_{\dosmash{\textrm{obs}}}}
\shortcut{\nobssn}{\snindex{N_{\dosmash{\textrm{obs}}}}}

\shortcut{\deltat}{\Delta\phase}
\shortcut{\deltatsn}{\snindex{\deltat}}

\newcommand{\snindexlabel}{\ensuremath{s}\xspace}
\newcommand{\snindex}[2][\snindexlabel]{#2^{#1}}
\newcommand{\obsindexlabel}{\ensuremath{i}\xspace}
\newcommand{\obsindex}{\snindex[\obsindexlabel]}
\newcommand{\snobsindexlabel}{\snindexlabel, \obsindexlabel}
\newcommand{\snobsindex}{\snindex[\snobsindexlabel]}

\newcommand{\lparamssn}{\snindex{\lparams}}
    \shortcut{\lparamsobs}{\hat{\lparams}}
    \newcommand{\lparamsobssn}{\snindex{\lparamsobs}}
\newcommand{\iglparamssn}{\igindex[\smash{\igindexlabel}]{\lparamssn}}

\newcommand{\datasn}{\snindex{\data}}
\newcommand{\datasnobs}{\varcomp{\snobsindex{\data}}}
\newcommand{\obsmeta}{\metadata_{\smash{\textrm{obs}}}}
\newcommand{\snmeta}{\metadata_{\smash{\textrm{\SN}}}}
\newcommand{\metadataobs}{\obsindex{\obsmeta}}
\newcommand{\metadatasn}{\snindex{\snmeta}}
\newcommand{\metadatasnobs}{\snobsindex{\obsmeta}}

\newcommand{\phasesnobs}{\snobsindex{\phase}}
\newcommand{\bandsnobs}{\snobsindex{\band}}
\newcommand{\ZPsnobs}{\snobsindex{\ZP}}
\newcommand{\gainsnobs}{\snobsindex{\gain}}
\newcommand{\srcratesnobs}{\snobsindex{\srcrate}}
\newcommand{\bgratesnobs}{\snobsindex{\bgrate}}
\shortcut{\fluxcalsnobs}{\snobsindex{\fluxcal}}
\shortcut{\fluxcalerrsnobs}{\snobsindex{\fluxcalerr}}

\shortcut{\bhmcovar}{\variable{x}}
    \newcommand{\bhmcovarsn}{\snindex{\bhmcovar}}
    \shortcut{\bhmcovarobs}{\hat{\bhmcovar}}
    \newcommand{\bhmcovarobssn}{\snindex{\bhmcovarobs}}

\shortcut{\trippcorr}{\variable{\alpha}}
\shortcut{\trippcovar}{\hat{\bhmcovar}}
\shortcut{\trippresid}{\epsilon}
\newcommand{\trippresidsn}{\snindex{\trippresid}}

\shortcut{\absmag}{M}
\shortcut{\appmag}{m}

\newcommand{\Msn}{\snindex{\absmag}}
\shortcut{\mobs}{\widehat{\appmag}}
\shortcut{\mobssn}{\snindex{\dosmash{\mobs}\vphantom{m}}}
\newcommand{\msn}{\snindex{\appmag}}
\newcommand{\zsn}{\snindex{\z}}
\shortcut{\zobs}{\hat{\z}}
\newcommand{\zobssn}{\snindex{\zobs}}
\newcommand{\zcsn}{\snindex{\zc}}
\shortcut{\zcobs}{\widehat{\zc}}
\newcommand{\zcobssn}{\snindex{\zcobs}}
\shortcut{\zpecobs}{\widehat{\zpec}}
\shortcut{\vpecobs}{\widehat{\vpec}}
\newcommand{\distmodsn}{\snindex{\distmod}}
\shortcut{\distmodobs}{\hat{\distmod}}
\newcommand{\distmodobssn}{\snindex{\distmodobs}}

\newcommand{\spectralfluxsn}{\snindex{\spectralflux}}

\shortcut{\Mo}{M_0}
\shortcut{\sigmares}{\sigma_{\smash{0}}}
\newcommand{\varres}{\sigmares^2}
\shortcut{\sigmaz}{\sigma_{\z}}
\newcommand{\varz}{\sigmaz^2}
\shortcut{\sigmazc}{\sigma_{\zc}}
\newcommand{\varzc}{\sigmazc^2}
\shortcut{\sigmadistmod}{\sigma_{\distmod}}
\newcommand{\vardistmod}{\sigmadistmod^2}
\shortcut{\covdistmod}{\hat{\varmatrix{C}}_{\distmod}}

% SALT
\newcommand{\saltf}{\spectralflux}
\shortcut{\npca}{N_{\textrm{PCA}}}
\newmathcommand{\pcaindexlabel}{i}
\newcommand{\pcaindex}[2][]{#2_{\ifblank{#1}{\smash{\pcaindexlabel}}{#1}}}
\newcommand{\saltfcomp}[1][]{\pcaindex[#1]{\saltf}}
\shortcut{\saltgenx}{x}
    \newcommand{\saltxcomp}[1][]{\pcaindex[#1]{\saltgenx}}
    \newcommand{\saltxcompsn}[1][\pcaindexlabel]{\snindex{\saltxcomp[\smash{#1}]}}
\newcommand{\saltx}{\saltxcomp[1]}
    \newcommand{\saltxsn}{\snindex{\saltx}}
    \shortcut{\saltxobs}{\hat{\saltgenx}_{\smash{1}}}
    \newcommand{\saltxobssn}{\snindex{\saltxobs}}
\newoperator{\saltcl}{CL}
\shortcut{\saltc}{c}
    \newcommand{\saltcsn}{\snindex{\saltc}}
    \shortcut{\saltcobs}{\hat{\saltc}}
    \newcommand{\saltcobssn}{\snindex{\saltcobs}}
\shortcut{\saltalpha}{\alpha}
\shortcut{\saltalphac}{\alpha_{\saltc}}
\shortcut{\saltbeta}{\beta}

\newcommand{\snintlabel}{\ensuremath{\mathrm{int}}\xspace}
\newcommand{\snextlabel}{\ensuremath{\mathrm{ext}}\xspace}
\newcommand{\snint}[2][\snintlabel]{#2_{#1}}
\newcommand{\Mint}{\snint{\absmag}}
    \newcommand{\Mintsn}{\snindex{\Mint}}
    \newcommand{\Mext}{\snint[\snextlabel]{\absmag}}
    \newcommand{\Mextsn}{\snindex{\Mext}}
\newcommand{\saltxint}{\snint{\saltgenx}}
    \newcommand{\saltxintsn}{\snindex{\saltxint}}
    \newcommand{\saltxext}{\snint[\snextlabel]{\saltgenx}}
    \newcommand{\saltxextsn}{\snindex{\saltxext}}
\newcommand{\saltcint}{\snint{\saltc}}
    \newcommand{\saltcintsn}{\snindex{\saltcint}}
    \newcommand{\saltcext}{\snint[\snextlabel]{\saltc}}
    \newcommand{\saltcextsn}{\snindex{\saltcext}}

% BAHAMAS
\newcommand{\bhmpriorsaltalpha}{\ensuremath{\Uniform(\num{0}, \num{1})}}
\newcommand{\bhmpriorsaltbeta}{\ensuremath{\Uniform(\num{0}, \num{4})}}
\newcommand{\bhmpriormeanMo}{\ensuremath{\Normal(\num{-19.3}, \num{2}^2)}}
\newcommand{\bhmpriorvarres}{\ensuremath{\InvGammaDist(\num{0.003}, \num{0.003})}}
\newcommand{\bhmpriormeansaltx}{\ensuremath{\Normal(\num{0}, \num{10}^2)}}
\newcommand{\bhmpriorstdsaltx}{\ensuremath{\log \Uniform(\num{e-5}, \num{e2})}}
\newcommand{\bhmpriormeansaltc}{\ensuremath{\Normal(\num{0}, \num{1}^2)}}
\newcommand{\bhmpriorstdsaltc}{\ensuremath{\log \Uniform(\num{e-5}, \num{e2})}}
\newcommand{\bhmpriorvarz}{\ensuremath{\InvGammaDist(\num{0.0003}, \num{0.0003})}}

\shortcut{\estzcsn}{\widehat{\snindex[\smash{\snindexlabel}]{\z_{\smash{\mathrm{c}}}}}}
\newmathcommand{\bhmpostzcsn}{\Normal(\estzcsn, \qty(1+\estzcsn)^2\varz)}

\newcommand{\Mosn}{\snindex{\Mo}}
\shortcut{\meanMo}{\bar{M}_0}
\newmathcommand{\priorMosn}{\Normal(\meanMo, \varres)}
\shortcut{\meansaltx}{\bar{\saltgenx}_1}
\shortcut{\stdsaltx}{R_{\smash{\saltx}}}
\newmathcommand{\priorsaltxsn}{\Normal(\meansaltx, \stdsaltx^2)}
\shortcut{\meansaltc}{\bar{\saltc}}
\shortcut{\stdsaltc}{R_{\smash{\saltc}}}
\newmathcommand{\priorsaltcsn}{\Normal(\meansaltc, \stdsaltc^2)}

\shortcut{\bhmobs}{\variable{y}}
\shortcut{\bhmobssn}{\snindex{\bhmobs}}
\shortcut{\datacovar}{\hat{\varmatrix{\Sigma}}}
\shortcut{\datacovarsn}{\snindex{\datacovar}}

% BAYESN
\newmathcommand{\priorbsnsigmadeltaM}{\HalfCauchy(0.1)}
\newmathcommand{\priormeanRv}{\Uniform(1.2, 5)}
\newmathcommand{\priorsigmaRv}{\HalfNormal(2^2)}
\newmathcommand{\priorbsntau}{\HalfCauchy(1)}

\shortcut{\bsndeltaM}{\var{M}}
\newcommand{\bsndeltaMsn}{\snindex{\bsndeltaM}}
\shortcut{\bsnmeandeltaM}{\mu_{\deltaM}}
\newcommand{\bsnsigmadeltaM}{\sigmares}
\newmathcommand{\priorbsndeltaM}{\Normal(0, \bsnsigmadeltaM^2)}

\shortcut{\bsne}{\variable{e}}
\newcommand{\bsnesn}{\snindex{\bsne}}

\shortcut{\bsnsigmae}{\variable{\sigma}_{\bsne}}
\shortcut{\bsnRe}{\varmatrix{R}_{\bsne}}
\shortcut{\bsnSigmae}{\varmatrix{\Sigma}_{\bsne}}
\newmathcommand{\priorbsne}{\Normal(\variable{0}, \bsnSigmae)}

\shortcut{\bsntheta}{\theta_{\smash{1}}}
\shortcut{\bsnthetasn}{\snindex{\bsntheta}}
\newmathcommand{\priorbsntheta}{\Normal(0, 1^2)}

\newcommand{\splinend}[3][2]{\ensuremath{\opbraces{\operatorname{Spline#1d}}(#2 ;\, #3)}}
\shortcut{\ngrid}{N_{\textrm{grid}}}
\newcommand{\gridindexlabel}{\textrm{g}\xspace}
\newcommand{\gridindex}[1]{#1_{\gridindexlabel}}

\shortcut{\bsngridphase}{\gridindex{\variable{\phase}}}
\shortcut{\bsngridwave}{\gridindex{\variable{\wave}}}
\newsubmathcommand{\bsnW}{}{W}
\newsubmathcommand{\bsngridW}{1}{\variable{\bsnW}}

\newcommand{\bsnE}{\trippresid}
\newcommand{\bsnEsn}{\snindex{\bsnE}}

% DUST
\shortcut{\Rv}{R_{\passband{V}}}
\newcommand{\Rvsn}{\snindex{\Rv}}
\shortcut{\meanRv}{\mu_{R}}
\shortcut{\sigmaRv}{\sigma_{R}}
\newmathcommand{\priorRv}{\Normal(\meanRv, \sigmaRv^2)}
\newmathcommand{\domainRv}{\interval[open right]{\num{1.2}}{\infty}}

\newcommand{\Edust}[2]{\ensuremath{E_{\passband{#1}-\passband{#2}}}}
\newcommand{\EBV}{\Edust{B}{V}}
    \newmathcommand{\EBVsn}{\snindex{\EBV}}
\newcommand{\Adust}[1]{\ensuremath{A_{\passband{#1}}}}
\shortcut{\Av}{A_{\passband{V}}}
    \newcommand{\Avsn}{\snindex{\Av}}
\shortcut{\bsntau}{\tau}
\newmathcommand{\priorAv}{\Exponential(\flatfrac{1}{\tau})}

\newcommand{\MWVsub}{\passband{V}, \textrm{MW}}
\newcommand{\smashedMWVsub}[1]{\begingroup%
    \let\oldMWVsub\MWVsub%
    \renewcommand{\MWVsub}{\smash{\oldMWVsub}}%
    #1%
\endgroup}
\shortcut{\MWRv}{R_{\MWVsub}}
\shortcut{\MWAv}{A_{\MWVsub}}
\newcommand{\MWAvsn}{\snindex{\MWAv}}
\shortcut{\MWAvobs}{\hat{A}_{\MWVsub}}
\newcommand{\MWAvobssn}{\snindex{\MWAvobs}}

\shortcut{\Fitzpatrick}{\operatorname{F99}}

% RATE
\DeclareSIUnit{\snrateunit}{\cubic\cosmoh\seventy \per\cubic\mega\parsec \per\year}
\shortcut{\snrate}{R}
\shortcut{\snratenull}{R_0}
\shortcut{\snrateexp}{\beta}
\shortcut{\snrateexphigh}{\gamma}
\shortcut{\snratezbreak}{\z_{\textrm{break}}}
\shortcut{\surveyduration}{T}
\newcommand{\surveyarea}{\solidangle}

% HOST
\shortcut{\ngal}{N_{\textrm{gal}}}

\newcommand{\hostindexlabel}{\ensuremath{h}\xspace}
\newcommand{\hostindex}[2][\hostindexlabel]{#2^{#1}}
\newcommand{\popindexlabel}{\ensuremath{i}\xspace}
\newcommand{\popindex}[2][\popindexlabel]{#2_{#1}}
\newcommand{\hostpopindexlabel}{\ensuremath{\hostindexlabel,\popindexlabel}\xspace}
\newcommand{\hostpopindex}[2][\hostpopindexlabel]{#2^{#1}}

\newcommand{\datagal}{\hostindex{\data}}

\newcommand{\zgal}{\hostindex{\z}}
\newcommand{\zcgal}{\hostindex{\zc}}
\newcommand{\tagegal}{\hostindex{\tage}}

\shortcut{\hparams}{\variable{g}}
    \newcommand{\hparamssn}{\snindex{\hparams}}
    \newcommand{\hparamsgal}{\hostindex{\hparams}}
\shortcut{\hparamsobs}{\hat{\hparams}}
    \newcommand{\hparamsobssn}{\snindex{\hparamsobs}}
    \newcommand{\hparamsobsgal}{\hostindex{\hparamsobs}}
\shortcut{\Mstar}{M_{*}}
    \newcommand{\Mstarsn}{\snindex{\Mstar}}
    \newcommand{\Mstargal}{\hostindex{\Mstar}}
    \shortcut{\Mstarobs}{\hat{M}_{*}}
    \newcommand{\Mstarobssn}{\snindex{\Mstarobs}}

\shortcut{\logMstar}{\mathcal{M}}
    \newcommand{\logMstarsn}{\snindex{\logMstar}}
    \newcommand{\logMstargal}{\hostindex{\logMstar}}
\shortcut{\Zstar}{Z_{*}}
    \newcommand{\Zstarsn}{\snindex{\Zstar}}
    \newcommand{\Zstargal}{\hostindex{\Zstar}}
\newmathcommand{\logZstarring}[1]{\lg\flatfrac{#1}{\si[unit-mode=math]{\Zsun}}}
\newmathcommand{\logZstar}{\logZstarring{\Zstar}}
    \newmathcommand{\logZstargal}{\logZstarring{\Zstargal}}
    \newmathcommand{\logZstarsn}{\logZstarring{\Zstarsn}}
\newcommand{\tstar}{\baseextensive{t}_{*}}
    \newcommand{\tstarsn}{\snindex{\tstar}}

\newcommand{\Msplit}{\Mstar^{\mathrm{split}}}
\shortcut{\Msplitindicator}{\varcomp{\trippcovar_{\smash{\Mhost}}}}
\shortcut{\Mstep}{\Delta\absmag}
\newcommand{\Msteploc}{\Mstar^{\smash{\mathrm{step}}\vphantom{\mathrm{t}}}}

\shortcut{\gammaMZ}{\gamma_{\Zstar}}
\shortcut{\gammaMt}{\gamma_{\tstar}}

\newcommand{\deltaM}{\bsndeltaM}
\newcommand{\deltaMsn}{\bsndeltaMsn}

% NN
\newoperator[\nncomp]{\SNEmbed}{SNEmbed}
\newoperator[\nncomp]{\SNHead}{SNHead}
\newoperator[\nncomp]{\AuxHead}{AuxHead}

\newcommand{\nndatasn}{\snindex{\nndata}}
\shortcut{\nnembsn}{\snindex{\nnvar{f}}}
\newcommand{\nnlparamssn}{\snindex{\nnlparams}}
\newcommand{\nnmetasn}{\snindex{\nnmeta}}
\shortcut{\nncosmoparams}{\nnvar{C}}


==> lib/extra/sn/slicsim.tex <==
\newcommand{\Source}{\texttt{Source}\xspace}
\newcommand{\ConstantSource}{\texttt{Constant\allowbreak Source}\xspace}
\newcommand{\Effect}{\texttt{Effect}\xspace}
\newcommand{\Extinction}{\texttt{Extinction}\xspace}
\newcommand{\Redshift}{\texttt{Redshift}\xspace}
\newcommand{\Distance}{\texttt{Distance}\xspace}
\newcommand{\CosmologicalDistance}{\texttt{Cosmological\allowbreak Distance}\xspace}
\newcommand{\Phaseshift}{\texttt{Phaseshift}\xspace}

==> lib/journals.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 5.2
%  and are compatible with the macros in the A&A document class
%  version 7.0
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package or the A&A document class and need to
%  resolve the macro definitions in the TeX/BibTeX entries returned by
%  the ADS abstract service.
%
%  If you plan not to use this file to resolve the journal macros
%  rather than the whole AAS TeX macro package, you should save the
%  file as ``aas_macros.sty'' and then include it in your LaTeX paper
%  by using a construct such as:
%	\documentstyle[11pt,aas_macros]{article}
%
%  For more information on the AASTeX and A&A packages, please see:
%       http://journals.aas.org/authors/aastex.html	
%       ftp://ftp.edpsciences.org/pub/aa/readme.html
%  For more information about ADS abstract server, please see:
%       http://adsabs.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).

\makeatletter
\let\jnl@style=\rm
\def\ref@jnl#1{{\jnl@style#1}}

\def\aj{\ref@jnl{AJ}}                   % Astronomical Journal
\def\actaa{\ref@jnl{Acta Astron.}}      % Acta Astronomica
\def\araa{\ref@jnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\ref@jnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\ref@jnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\ref@jnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\ref@jnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\ref@jnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\ref@jnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\ref@jnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\ref@jnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\ref@jnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\ref@jnl{BAAS}}               % Bulletin of the AAS
\def\bac{\ref@jnl{Bull. astr. Inst. Czechosl.}}
% Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{\ref@jnl{Chinese Astron. Astrophys.}}
% Chinese Astronomy and Astrophysics
\def\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}
% Chinese Journal of Astronomy and Astrophysics
\def\icarus{\ref@jnl{Icarus}}           % Icarus
\def\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}
% Journal of Cosmology and Astroparticle Physics
\def\jrasc{\ref@jnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\ref@jnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\ref@jnl{MNRAS}}             % Monthly Notices of the RAS
\def\na{\ref@jnl{New A}}                % New Astronomy
\def\nar{\ref@jnl{New A Rev.}}          % New Astronomy Review
\def\pra{\ref@jnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\ref@jnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\ref@jnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\ref@jnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\ref@jnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\ref@jnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasa{\ref@jnl{PASA}}               % Publications of the Astron. Soc. of Australia
\def\pasp{\ref@jnl{PASP}}               % Publications of the ASP
\def\pasj{\ref@jnl{PASJ}}               % Publications of the ASJ
\def\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
% Revista Mexicana de Astronomia y Astrofisica
\def\qjras{\ref@jnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\ref@jnl{S\&T}}             % Sky and Telescope
\def\solphys{\ref@jnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\ref@jnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\ref@jnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\ref@jnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\ref@jnl{Nature}}              % Nature
\def\iaucirc{\ref@jnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\ref@jnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}
% Astrophysics Space Physics Research
\def\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}} 
% Bulletin Astronomical Institute of the Netherlands
\def\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\ref@jnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\ref@jnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\ref@jnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}
% Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}
% Mem. Societa Astronomica Italiana
\def\nphysa{\ref@jnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\ref@jnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\ref@jnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\ref@jnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\ref@jnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
\makeatother

==> lib/mypgf/ellipse.tex <==
\ifLuaTeX\usepackage{luacode}\fi

%https://tex.stackexchange.com/questions/95470/parallel-loop-python-like-zip-in-tikz
\makeatletter
\protected\def\zip{%
	\begingroup
	\@ifstar{\def\cnta{1}\@zip}
	{\def\cnta{0}\@zip}%
}
\def\@zip#1#2#3#4{%
	\def\tempa##1##2{%
		\edef##2{%
			\ifnum\cnta=\@ne\else\expandafter\@firstoftwo\fi
			\unexpanded\expandafter{##1}%
		}%
	}%
	\tempa{#2}\tempb\tempa{#3}\tempa
	\def\cnta{0}\def#4{}%
	\foreach \x in \tempb{%
		\xdef\cnta{\the\numexpr\cnta+1}%
		\gdef\cntb{0}%
		\foreach \y in \tempa{%
			\xdef\cntb{\the\numexpr\cntb+1}%
			\ifnum\cntb=\cnta\relax
			\xdef#4{#4\ifx#4\empty\else,\fi\x#1\y}%
			\breakforeach
			\fi
		}%
	}%
	\endgroup
}
\makeatother


% ELLIPSE
% -------
\ifLuaTeX
\begin{luacode*}
	function sign(a)
		return (a > 0 and 1) or (a == 0 and 0) or -1
	end

	function ow(w, h, theta, t)
		return theta == 0 and w or w == h and w*math.sqrt(2*t^2 + 2*math.sqrt(t^4 - 2*t^2 + 1) + 2)/2 or  math.sqrt(h^2*t^2*math.cos(theta)^2/2 + h^2*math.sin(theta)^2/2 + t^2*w^2*math.sin(theta)^2/2 + w^2*math.cos(theta)^2/2 + math.sqrt(-4*h^2*t^2*w^2 + (h^2*t^2*math.cos(theta)^2 + h^2*math.sin(theta)^2 + t^2*w^2*math.sin(theta)^2 + w^2*math.cos(theta)^2)^2)/2)
	end
	function oh(w, h, theta, t)
		return theta == 0 and h or w == h and w*math.sqrt(2*t^2 - 2*math.sqrt(t^4 - 2*t^2 + 1) + 2)/(2*t) or math.sqrt(h^2*t^2*math.cos(theta)^2/2 + h^2*math.sin(theta)^2/2 + t^2*w^2*math.sin(theta)^2/2 + w^2*math.cos(theta)^2/2 - math.sqrt(-4*h^2*t^2*w^2 + (h^2*t^2*math.cos(theta)^2 + h^2*math.sin(theta)^2 + t^2*w^2*math.sin(theta)^2 + w^2*math.cos(theta)^2)^2)/2)/t
	end
	function oa(w, h, theta, t)
		return theta == 0 and 0 or w == h and 0 or math.atan2(sign(theta)/math.sqrt(4*t^2*math.abs((h^2 - w^2)*math.sin(theta)*math.cos(theta)/(h^2*t^2*math.cos(theta)^2 - h^2*math.sin(theta)^2 + t^2*w^2*math.sin(theta)^2 - w^2*math.cos(theta)^2 + math.sqrt(h^4*t^4*math.cos(theta)^4 - h^4*t^2*(math.cos(4*theta) - 1)/4 + h^4*math.sin(theta)^4 - h^2*t^4*w^2*(math.cos(4*theta) - 1)/4 + 2*h^2*t^2*w^2*math.sin(theta)^4 + 2*h^2*t^2*w^2*math.cos(theta)^4 - 4*h^2*t^2*w^2 - h^2*w^2*(math.cos(4*theta) - 1)/4 + t^4*w^4*math.sin(theta)^4 - t^2*w^4*(math.cos(4*theta) - 1)/4 + w^4*math.cos(theta)^4)))^2 + 1), 1/math.sqrt(4*t^2*math.abs((h^2 - w^2)*math.sin(theta)*math.cos(theta)/(-h^2*t^2*math.cos(theta)^2 + h^2*math.sin(theta)^2 - t^2*w^2*math.sin(theta)^2 + w^2*math.cos(theta)^2 + math.sqrt(h^4*t^4*math.cos(theta)^4 - h^4*t^2*(math.cos(4*theta) - 1)/4 + h^4*math.sin(theta)^4 - h^2*t^4*w^2*(math.cos(4*theta) - 1)/4 + 2*h^2*t^2*w^2*math.sin(theta)^4 + 2*h^2*t^2*w^2*math.cos(theta)^4 - 4*h^2*t^2*w^2 - h^2*w^2*(math.cos(4*theta) - 1)/4 + t^4*w^4*math.sin(theta)^4 - t^2*w^4*(math.cos(4*theta) - 1)/4 + w^4*math.cos(theta)^4)))^2 + 1))
	end

	function owm(a, b, c, t)
		return math.sqrt((a + b*t^2 - math.sqrt((a-b*t^2)^2 + 4*c^2*t^2))/2)
	end
	function ohm(a, b, c, t)
		return math.sqrt((a + b*t^2 + math.sqrt((a-b*t^2)^2 + 4*c^2*t^2))/2) / t
	end
	function oam(a, b, c, t)
		return c == 0 and 0 or math.atan2(
			1,
			(a - b*t^2 - math.sqrt((a-b*t^2)^2 + 4*c^2*t^2))/(2*c*t)
		)
	end
\end{luacode*}
\fi

\newcommand{\plotoneellipse}[5][]{
	\path[#1] (#2) circle[x radius={#3}, y radius={#4}, rotate={#5}];
}

\newcommand{\getdxdy}[1]{\pgfmathsetmacro{#1}{(\pgfkeysvalueof{/pgfplots/height} / \pgfkeysvalueof{/pgfplots/width}) * (\pgfkeysvalueof{/pgfplots/xmax} - \pgfkeysvalueof{/pgfplots/xmin}) / (\pgfkeysvalueof{/pgfplots/ymax} - \pgfkeysvalueof{/pgfplots/ymin})}}


\newcommand{\doplotellipse}[8]{
	\getdxdy{\t}
	\def\w{\directlua{tex.print(#6(#3, #4, #5, \t))}}
	\def\h{\directlua{tex.print(#7(#3, #4, #5, \t))}}
	\def\a{\directlua{tex.print(#8(#3, #4, #5, \t) * 180 / math.pi)}}

	\expandafter\pgfplotsforeach\expandafter{\loopvars}{\zipped}{
		\noexpand\plotoneellipse[#1, \nargs]{#2}{\ns * \w}{\ns * \h}{\a}
	}
}

\NewDocumentCommand{\plotellipseabc}{O{} r() m m m O{1} o}{
	\IfNoValueTF{#7}
	{\def\zipped{#6} \def\loopvars{\ns} \def\nargs{}}
	{\zip{/}{#6}{#7}\zipped \def\loopvars{\ns/\nargs}}

	\doplotellipse{#1}{#2}{#3}{#4}{#5}{owm}{ohm}{oam}
}

\NewDocumentCommand{\plotellipse}{O{} r() m m m O{1} o}{
	\IfNoValueTF{#7}
	{\def\zipped{#6} \def\loopvars{\ns} \def\nargs{}}
	{\zip{/}{#6}{#7}\zipped \def\loopvars{\ns/\nargs}}

	\doplotellipse{#1}{#2}{#3}{#4}{#5 * math.pi / 180}{ow}{oh}{oa}
}


==> lib/mypgf/utils.tex <==
\pgfkeys{
	/tikz/the color/.initial={},
	/tikz/color/.forward to=/tikz/the color,
}

% https://tex.stackexchange.com/questions/99315/specific-error-bars-in-pgfplots-possible
\newcounter{marknumber}
\pgfplotsset{
    error bars/every nth mark/.style={
        /pgfplots/execute at begin plot visualization={\setcounter{marknumber}{0}},
		/pgfplots/error bars/draw error bar/.prefix code={
			\pgfmathtruncatemacro\marknumbercheck{mod(floor(\themarknumber/2),#1)}
			\ifnum\marknumbercheck=0
			\else
			\begin{scope}[opacity=0]
				\fi
			},
			/pgfplots/error bars/draw error bar/.append code={
				\ifnum\marknumbercheck=0
				\else
			\end{scope}
			\fi
			\stepcounter{marknumber}
		}
	},
}

% https://tex.stackexchange.com/a/26386/205294
\makeatletter
\tikzset{
	use path for main/.code={%
		\tikz@addmode{%
			\expandafter\pgfsyssoftpath@setcurrentpath\csname tikz@intersect@path@name@#1\endcsname
		}%
	},
	use path for actions/.code={%
		\expandafter\def\expandafter\tikz@preactions\expandafter{\tikz@preactions\expandafter\let\expandafter\tikz@actions@path\csname tikz@intersect@path@name@#1\endcsname}%
	},
	use path/.style={%
		use path for main=#1,
		use path for actions=#1,
	}
}

%https://tex.stackexchange.com/a/38500
\def\calcLength(#1,#2)#3{%
	\pgfpointdiff{\pgfpointanchor{#1}{center}}%
	{\pgfpointanchor{#2}{center}}%
	\pgf@xa=\pgf@x%
	\pgf@ya=\pgf@y%
	\FPeval\@temp@a{\pgfmath@tonumber{\pgf@xa}}%
	\FPeval\@temp@b{\pgfmath@tonumber{\pgf@ya}}%
	\FPeval\@temp@sum{(\@temp@a*\@temp@a+\@temp@b*\@temp@b)}%
	\FProot{\FPMathLen}{\@temp@sum}{2}%
	\FPround\FPMathLen\FPMathLen5\relax
	\global\expandafter\edef\csname #3\endcsname{\FPMathLen}
}

\makeatother

\tikzmath{%
	function randn(\x) {
		return \x * sin(360*rnd)*sqrt(-2*ln(rnd));
	};
	function gaussian(\x) {
		return exp(- ((\x)^2) / 2);
	};
}

\newif\ifcolorbarishorizontal
\pgfplotsset{
    log ticks with fixed point style/.initial={fixed relative, precision=3},
    log xticks with fixed point/.default/.forward to={/pgfplots/log ticks with fixed point style},
	log xticks with fixed point/.style={
		xticklabel={
			\pgfkeys{/pgf/fpu=true}
			\pgfmathparse{exp(\tick)}%
			\pgfmathprintnumber[#1]{\pgfmathresult}
			\pgfkeys{/pgf/fpu=false}
		}
	},
    log yticks with fixed point/.default/.forward to={/pgfplots/log ticks with fixed point style},
	log yticks with fixed point/.style={
		yticklabel={
			\pgfkeys{/pgf/fpu=true}
			\pgfmathparse{exp(\tick)}%
			\pgfmathprintnumber[#1]{\pgfmathresult}
			\pgfkeys{/pgf/fpu=false}
		}
	},
    inner aligned xticklabels top/.style={
        xticklabel style={
            anchor={\ifnum\ticknum=0 south west\else\ifnum\ticknum=#1 south east\else south\fi\fi},
            inner xsep=0pt
        }},
	inner aligned xticklabels/.style={
		xticklabel style={
			anchor={\ifnum\ticknum=0 north west\else\ifnum\ticknum=#1 north east\else north\fi\fi},
			inner xsep=0pt
		}},
	inner aligned yticklabels/.style={
		yticklabel style={
			anchor={\ifnum\ticknum=0 south east\else\ifnum\ticknum=#1 north east\else east\fi\fi},
			inner ysep=0pt
		}},
    inner aligned yticklabels/.style={
        yticklabel style={
        anchor={\ifnum\ticknum=0 south west\else\ifnum\ticknum=#1 north west\else west\fi\fi},
        inner ysep=0pt
    }},
    % TIGHT LAYOUT
    tight layout*/.style n args={3}{
        scale only axis,
        width/.evaluated={1/(#1)*(#2) - (#1-1)/(#1)*(#3)},
    },
	tight layout/.style={tight layout*={#1}{\linewidth}{\pgfkeysvalueof{/pgfplots/group/horizontal sep}}},
	same axis lims/.style 2 args={
		xmin={#1}, xmax={#2},
		ymin={#1}, ymax={#2},
	},
    % HISTOGRAM
	histogram/.style={
		hist/data filter/.code={\pgfmathparse{and(##1 > \pgfkeysvalueof{/pgfplots/hist/data min}, ##1 < \pgfkeysvalueof{/pgfplots/hist/data max}) ? ##1 : inf}}
	},
	% VARIOUS
	extent/.code={
		\pgfplotsset{xmin={-#1}, xmax={#1}, ymin={-#1}, ymax={#1}}
	},
	colorbar is horizontal/.is if=colorbarishorizontal,
	colorbar label/.code={
		\ifcolorbarishorizontal
			\pgfplotsset{colorbar style={xlabel=#1}}
		\else
			\pgfplotsset{colorbar style={ylabel=#1}}
		\fi
	},
	plot graphics/!src/.code={
		\pgfplotsset{
			plot graphics/lowlevel draw/.code 2 args={\includegraphics[\pgfkeysvalueof{/pgfplots/plot graphics/includegraphics},width=##1,height=##2] {#1}}
		}
	},
	matrix colormesh/.style = {
		matrix plot*, point meta=explicit, line join=miter
	},
	/tikz/credible region/.style={/tikz/draw/.expanded={\pgfkeysvalueof{/tikz/the color}!50!black}, fill},
	/tikz/1 sigma region/.style={thin, fill opacity=0.95, credible region},
	/tikz/2 sigma region/.style={semithick, fill opacity=0.6, credible region},
	ellipses* legend/.style 2 args={
		/pgfplots/legend image code/.code={
			\begin{scope}[shift={(#1,0)}]
				\path[##1, 2 sigma region] (0,0)
				circle[x radius=#1, y radius=#2];
				\path[##1, 1 sigma region] (0,0)
				circle[x radius={#1/2}, y radius={#2/2}];
			\end{scope}
		}
	},
	ellipses legend/.style={ellipses* legend={0.3cm}{0.1cm}},
}

% Thanks, egreg! https://tex.stackexchange.com/a/603677/205294
\ExplSyntaxOn
\NewDocumentCommand{\addplotnamedtable}{oO{}m}{\IfNoValueTF{#1}{
	\use:e { \exp_not:n { \addplot table~[#2] } { \exp_not:c { #3 } } }
}{
	\use:e { \exp_not:n { \addplot [#1]~table~[#2] } { \exp_not:c { #3 } } }
}}
\ExplSyntaxOff

\NewDocumentCommand{\axhline}{O{} m O{0} O{1} O{0}}{
	\draw[/pgfplots/every axis plot, #1] ({{rel axis cs:#3,0}} |- {{axis cs:#5,#2}}) -- ({{rel axis cs:#4,0}} |- {{axis cs:#5,#2}})
}
\NewDocumentCommand{\axvline}{O{} m O{0} O{1} O{0}}{
	\draw[/pgfplots/every axis plot, #1] ({{rel axis cs:0,#3}} -| {{axis cs:#2,#5}}) -- ({{rel axis cs:0,#4}} -| {{axis cs:#2,#5}})
}
\newcommand{\adddiagonallinex}[1][]{\draw[/pgfplots/every axis plot, #1] (\pgfkeysvalueof{/pgfplots/xmin}, \pgfkeysvalueof{/pgfplots/xmin}) -- (\pgfkeysvalueof{/pgfplots/xmax}, \pgfkeysvalueof{/pgfplots/xmax});}
\newcommand{\adddiagonalline}{\adddiagonallinex}

\newcommand{\pgfplotsforeach}[4][]{\foreach #2 [#1] in #3 {\edef\temp{#4}\temp}}
\newcommand{\pgfplotsforeachcommand}[3]{\foreach #1 in #2 {\edef\temp{\noexpand#3{#1}}\temp}}


\newcommand{\drawnode}[2][]{\draw[#1] (#2.south west) rectangle (#2.north east);}
\NewDocumentCommand{\labelPoint}{O{} r() m}{\tkzDrawPoint[\globalblackcolor](#2)\tkzLabelPoint[\globalblackcolor, #1](#2){#3}}


==> lib/patch/aastex.tex <==
% https://tex.stackexchange.com/a/742761/205294
\makeatletter
\pretocmd\@sect{\def\@currentcounter{#1}}{}{\fail}
\makeatother

\let\tablenum\relax
\AtBeginDocument{\let\tabular\savetabular}

\makeatletter
\let\switch@array\relax
\makeatother



==> lib/patch/foreach.tex <==
\makeatletter
\def\tikz@lib@fit@scan{%
	\pgfutil@ifnextchar\pgf@stop{\pgfutil@gobble}{%
		\pgfutil@ifnextchar\foreach{\tikz@lib@fit@scan@handle@foreach}{%
			\tikz@scan@one@point\tikz@lib@fit@scan@handle}}}
\def\tikz@lib@fit@scan@handle@foreach\foreach#1in#2#3{%
	\foreach #1 in {#2}
	{\tikz@scan@one@point\tikz@lib@fit@scan@handle@foreach@#3}
	\tikz@lib@fit@scan}
\def\tikz@lib@fit@scan@handle@foreach@#1{%
	\iftikz@shapeborder
	\tikz@lib@fit@adjust{%
		\pgfpointanchor{\tikz@shapeborder@name}{west}}%
	\tikz@lib@fit@adjust{%
		\pgfpointanchor{\tikz@shapeborder@name}{east}}%
	\tikz@lib@fit@adjust{%
		\pgfpointanchor{\tikz@shapeborder@name}{north}}%
	\tikz@lib@fit@adjust{%
		\pgfpointanchor{\tikz@shapeborder@name}{south}}%
	\else
	\tikz@lib@fit@adjust{#1}%
	\fi
	\global\pgf@xa=\pgf@xa
	\global\pgf@ya=\pgf@ya
	\global\pgf@xb=\pgf@xb
	\global\pgf@yb=\pgf@yb}
\makeatletter

==> lib/patch/mnras.tex <==
\makeatletter
\AtEndPreamble{
	% This empirically works...
	\setlength\textwidth{\SFB@measure}
}
\AfterEndPreamble{
	\label{firstpage}
	\pagerange{\pageref{firstpage}--\pageref{lastpage}}

	\maketitle
}
\AtEndDocument{
	\bsp
	\label{lastpage}
}
\makeatother


==> lib/shortcuts/dummy.tex <==
\makeatletter
% https://tex.stackexchange.com/a/449965
\newcommand {\crefcustom}[2]{\csname cref@#1@format\endcsname{#2}{}{}}
\newcommand {\Crefcustom}[2]{\csname Cref@#1@format\endcsname{#2}{}{}}

% https://tex.stackexchange.com/a/346255
\newcommand{\dummylabel}[3][equation]{\protected@edef\cref@currentlabel{[#1][0][0]#3}\label[#1]{#2}}
\newcommand{\crefext}{\cref*}

\makeatother


\newcommand{\SIDEreal}{S\Rnum{1}DE-real}
\newcommand{\SICRET}{S\Rnum{1}CRET}
\newcommand{\SimSIMS}{SimS\Rnum{1}MS}
\newcommand{\STARNRE}{STAR NRE}
\newcommand{\RESSET}{RESSET\xspace}
\newcommand{\CIGARS}{CIGaRS\xspace}
\defcitealias{Karchev-ptcosmo}{AADcosmo}
\defcitealias{Karchev-sicret}{\SICRET}
\defcitealias{Karchev-sidereal}{\SIDEreal}
\defcitealias{Karchev-simsims}{\SimSIMS}
\defcitealias{Karchev-starnre}{\STARNRE}


\AfterEndPreamble{
	\dummylabel[figure]{ext:Bishop_2006:fig:mode-seeking}{10.2}

	\dummylabel[subsection]{ext:EuCAPT_2021:sec:vi}{11.3.2}
	\dummylabel[subsection]{ext:EuCAPT_2021:sec:sbi}{11.3.3}

    \dummylabel[subsection]{ext:Karchev-vigp:sec:pmvn}{4.2}

	\dummylabel[section]{ext:Karchev-sicret:sec:tmnre}{3}
	\dummylabel[subsection]{ext:Karchev-sicret:sec:validation}{3.4}
	\dummylabel[figure]{ext:Karchev-sicret:fig:nn-arch}{2}
	\dummylabel[figure]{ext:Karchev-sicret:fig:freqcal}{3}
	\dummylabel[figure]{ext:Karchev-sicret:fig:bias}{4}

    \dummylabel[subsection]{ext:Karchev-sidereal:sec:redshift}{2.3}

    \dummylabel[subsection]{ext:Karchev-starnre:sec:detprob}{3.2}
    \dummylabel[appendix]{ext:Karchev-starnre:sec:cancel}{A}
}


==> lib/utils/utils.tex <==
\usepackage{pdftexcmds}

\makeatletter
% Expand #1 once before comparing it to #2
\newcommand*{\strcmp}[2]{%
	\expandafter\pdf@strcmp\expandafter{#1}{#2}%
}
\makeatother

% https://tex.stackexchange.com/a/23491/205294
\newcommand{\rnum}[1]{\romannumeral#1\relax}
\newcommand{\Rnum}[1]{\uppercase\expandafter{\romannumeral#1\relax}}

\newcommand{\dcancel}[2][0pt]{\tikz{\node[inner sep={#1}] (a) {#2}; \draw (a.south west)--(a.north east);}}

\newsavebox\commabox
\sbox{\commabox}{,}
\newlength\commalength
\newcommand{\commasup}{%
	\setlength\commalength{\wd\commabox}%
	,\kern-\commalength\textsuperscript}


\newcommand{\eosspace}{\spacefactor\sfcode`.\relax\xspace}
\newcommand{\magicperiod}[1]{\rlap{.}#1\eosspace}

\makeatletter
% https://tex.stackexchange.com/a/86717
% takes 2 arguments: #1<- cite-key, #2<- link-text
\newcommand*{\hypercite}[1]{\hyper@link{cite}{cite.#1}}
\makeatother


==> plotdata/hd.tex <==
\pgfkeys{,
/private/hd/.cd,
H0/us/.initial={71.60026431083679},
dM/us/.initial={0.0004520416259765625},
H0/Planck/.initial={67.4},
dM/Planck/.initial={0.13127364482120285},
H0/SH0ES/.initial={73},
dM/SH0ES/.initial={-0.04204117310447586},
h/.initial={0.7160026431083679},
mean_c/.initial={-0.07924097776412964},
sigma_c/.initial={0.035896360874176025},
}

==> plotdata/masses.tex <==
\pgfkeys{,
/private/masses/.cd,
full/range/.initial={7.338:11.413},
full/hist/.initial={(7.338, 0.0486318) (7.55247, 0.0486318) (7.55247, 0.0364739) (7.76695, 0.0364739) (7.76695, 0.0486318) (7.98142, 0.0486318) (7.98142, 0.0486318) (8.19589, 0.0486318) (8.19589, 0.0547108) (8.41037, 0.0547108) (8.41037, 0.0851057) (8.62484, 0.0851057) (8.62484, 0.103343) (8.83932, 0.103343) (8.83932, 0.127659) (9.05379, 0.127659) (9.05379, 0.249238) (9.26826, 0.249238) (9.26826, 0.35866) (9.48274, 0.35866) (9.48274, 0.249238) (9.69721, 0.249238) (9.69721, 0.455923) (9.91168, 0.455923) (9.91168, 0.632214) (10.1262, 0.632214) (10.1262, 0.516713) (10.3406, 0.516713) (10.3406, 0.607898) (10.5551, 0.607898) (10.5551, 0.516713) (10.7696, 0.516713) (10.7696, 0.346502) (10.9841, 0.346502) (10.9841, 0.12158) (11.1985, 0.12158) (11.1985, 0.0547108) (11.413, 0.0547108)},
full/kde/.initial={(7.338, 0.0253446) (7.35848, 0.0269701) (7.37895, 0.0284961) (7.39943, 0.029902) (7.41991, 0.0311705) (7.44039, 0.032289) (7.46086, 0.0332502) (7.48134, 0.0340523) (7.50182, 0.0346996) (7.5223, 0.0352024) (7.54277, 0.0355762) (7.56325, 0.0358419) (7.58373, 0.0360242) (7.60421, 0.0361508) (7.62468, 0.0362512) (7.64516, 0.0363552) (7.66564, 0.0364913) (7.68612, 0.0366857) (7.70659, 0.0369606) (7.72707, 0.0373336) (7.74755, 0.0378167) (7.76803, 0.0384158) (7.7885, 0.0391305) (7.80898, 0.0399548) (7.82946, 0.040877) (7.84993, 0.0418813) (7.87041, 0.0429484) (7.89089, 0.0440571) (7.91137, 0.0451854) (7.93184, 0.0463124) (7.95232, 0.0474189) (7.9728, 0.048489) (7.99328, 0.0495111) (8.01375, 0.0504779) (8.03423, 0.0513873) (8.05471, 0.0522421) (8.07519, 0.05305) (8.09566, 0.0538225) (8.11614, 0.0545749) (8.13662, 0.0553248) (8.1571, 0.0560914) (8.17757, 0.0568945) (8.19805, 0.0577535) (8.21853, 0.0586865) (8.23901, 0.0597095) (8.25948, 0.0608362) (8.27996, 0.0620768) (8.30044, 0.0634385) (8.32091, 0.0649251) (8.34139, 0.0665369) (8.36187, 0.0682712) (8.38235, 0.0701227) (8.40282, 0.0720837) (8.4233, 0.0741448) (8.44378, 0.0762955) (8.46426, 0.0785249) (8.48473, 0.0808225) (8.50521, 0.0831787) (8.52569, 0.0855856) (8.54617, 0.0880378) (8.56664, 0.0905327) (8.58712, 0.0930708) (8.6076, 0.0956568) (8.62808, 0.0982991) (8.64855, 0.10101) (8.66903, 0.103806) (8.68951, 0.106706) (8.70998, 0.109735) (8.73046, 0.112916) (8.75094, 0.116278) (8.77142, 0.119849) (8.79189, 0.123655) (8.81237, 0.127725) (8.83285, 0.132081) (8.85333, 0.136747) (8.8738, 0.141738) (8.89428, 0.147066) (8.91476, 0.152736) (8.93524, 0.158747) (8.95571, 0.16509) (8.97619, 0.171747) (8.99667, 0.178693) (9.01715, 0.185895) (9.03762, 0.19331) (9.0581, 0.200888) (9.07858, 0.208572) (9.09906, 0.216301) (9.11953, 0.224005) (9.14001, 0.231615) (9.16049, 0.23906) (9.18096, 0.246269) (9.20144, 0.253178) (9.22192, 0.259726) (9.2424, 0.265865) (9.26287, 0.271558) (9.28335, 0.276781) (9.30383, 0.281529) (9.32431, 0.285814) (9.34478, 0.289668) (9.36526, 0.29314) (9.38574, 0.296301) (9.40622, 0.299238) (9.42669, 0.302053) (9.44717, 0.304858) (9.46765, 0.307776) (9.48813, 0.310932) (9.5086, 0.314449) (9.52908, 0.318446) (9.54956, 0.323029) (9.57004, 0.32829) (9.59051, 0.334301) (9.61099, 0.34111) (9.63147, 0.348742) (9.65194, 0.357193) (9.67242, 0.366433) (9.6929, 0.376406) (9.71338, 0.38703) (9.73385, 0.398203) (9.75433, 0.409804) (9.77481, 0.421698) (9.79529, 0.43374) (9.81576, 0.445783) (9.83624, 0.457681) (9.85672, 0.469293) (9.8772, 0.480489) (9.89767, 0.491154) (9.91815, 0.501189) (9.93863, 0.510516) (9.95911, 0.51908) (9.97958, 0.526844) (10.0001, 0.533795) (10.0205, 0.53994) (10.041, 0.545303) (10.0615, 0.549922) (10.082, 0.55385) (10.1024, 0.557147) (10.1229, 0.559878) (10.1434, 0.56211) (10.1639, 0.563907) (10.1844, 0.56533) (10.2048, 0.566431) (10.2253, 0.567252) (10.2458, 0.567825) (10.2663, 0.568171) (10.2867, 0.568295) (10.3072, 0.568194) (10.3277, 0.56785) (10.3482, 0.567238) (10.3687, 0.566321) (10.3891, 0.565057) (10.4096, 0.563398) (10.4301, 0.561291) (10.4506, 0.558685) (10.471, 0.555524) (10.4915, 0.551755) (10.512, 0.547329) (10.5325, 0.542198) (10.5529, 0.536321) (10.5734, 0.52966) (10.5939, 0.522184) (10.6144, 0.51387) (10.6349, 0.504702) (10.6553, 0.494671) (10.6758, 0.483779) (10.6963, 0.472037) (10.7168, 0.459467) (10.7372, 0.4461) (10.7577, 0.43198) (10.7782, 0.417163) (10.7987, 0.401713) (10.8192, 0.385709) (10.8396, 0.369237) (10.8601, 0.352391) (10.8806, 0.335274) (10.9011, 0.317992) (10.9215, 0.300654) (10.942, 0.283371) (10.9625, 0.26625) (10.983, 0.249393) (11.0035, 0.232896) (11.0239, 0.216848) (11.0444, 0.201325) (11.0649, 0.186393) (11.0854, 0.172104) (11.1058, 0.158499) (11.1263, 0.145605) (11.1468, 0.133439) (11.1673, 0.122005) (11.1877, 0.111298) (11.2082, 0.101304) (11.2287, 0.0920019) (11.2492, 0.0833666) (11.2697, 0.0753678) (11.2901, 0.0679734) (11.3106, 0.06115) (11.3311, 0.054864) (11.3516, 0.0490829) (11.372, 0.0437753) (11.3925, 0.0389115) (11.413, 0.0344638)},
late/range/.initial={8.509:11.218},
late/hist/.initial={(8.509, 0.0210475) (8.71738, 0.0210475) (8.71738, 0.0420949) (8.92577, 0.0420949) (8.92577, 0) (9.13415, 0) (9.13415, 0.210475) (9.34254, 0.210475) (9.34254, 0.315712) (9.55092, 0.315712) (9.55092, 0.189427) (9.75931, 0.189427) (9.75931, 0.589329) (9.96769, 0.589329) (9.96769, 0.652471) (10.1761, 0.652471) (10.1761, 0.862945) (10.3845, 0.862945) (10.3845, 0.694566) (10.5928, 0.694566) (10.5928, 0.715613) (10.8012, 0.715613) (10.8012, 0.399902) (11.0096, 0.399902) (11.0096, 0.105237) (11.218, 0.105237)},
late/kde/.initial={(8.509, 0.0121451) (8.52261, 0.0124495) (8.53623, 0.0127374) (8.54984, 0.0130151) (8.56345, 0.0132902) (8.57707, 0.0135709) (8.59068, 0.013866) (8.60429, 0.0141847) (8.6179, 0.0145361) (8.63152, 0.0149287) (8.64513, 0.0153709) (8.65874, 0.0158699) (8.67236, 0.0164323) (8.68597, 0.0170633) (8.69958, 0.0177675) (8.7132, 0.0185483) (8.72681, 0.0194081) (8.74042, 0.0203492) (8.75404, 0.0213735) (8.76765, 0.022483) (8.78126, 0.0236803) (8.79487, 0.0249694) (8.80849, 0.0263553) (8.8221, 0.0278455) (8.83571, 0.0294494) (8.84933, 0.0311792) (8.86294, 0.03305) (8.87655, 0.0350796) (8.89017, 0.0372888) (8.90378, 0.0397009) (8.91739, 0.0423415) (8.93101, 0.0452377) (8.94462, 0.048418) (8.95823, 0.051911) (8.97184, 0.0557444) (8.98546, 0.0599447) (8.99907, 0.0645353) (9.01268, 0.0695363) (9.0263, 0.0749625) (9.03991, 0.0808231) (9.05352, 0.0871207) (9.06714, 0.0938499) (9.08075, 0.100997) (9.09436, 0.108541) (9.10797, 0.116448) (9.12159, 0.12468) (9.1352, 0.133185) (9.14881, 0.141906) (9.16243, 0.150777) (9.17604, 0.159723) (9.18965, 0.168665) (9.20327, 0.17752) (9.21688, 0.186202) (9.23049, 0.194622) (9.24411, 0.202695) (9.25772, 0.210339) (9.27133, 0.217475) (9.28494, 0.224036) (9.29856, 0.229961) (9.31217, 0.235205) (9.32578, 0.239733) (9.3394, 0.243528) (9.35301, 0.246591) (9.36662, 0.248938) (9.38024, 0.250604) (9.39385, 0.251643) (9.40746, 0.252127) (9.42108, 0.252142) (9.43469, 0.251792) (9.4483, 0.251193) (9.46191, 0.250471) (9.47553, 0.249762) (9.48914, 0.249204) (9.50275, 0.248939) (9.51637, 0.249107) (9.52998, 0.249844) (9.54359, 0.251276) (9.55721, 0.253519) (9.57082, 0.256674) (9.58443, 0.260826) (9.59805, 0.266042) (9.61166, 0.272369) (9.62527, 0.27983) (9.63888, 0.28843) (9.6525, 0.298148) (9.66611, 0.308946) (9.67972, 0.320762) (9.69334, 0.333518) (9.70695, 0.347117) (9.72056, 0.36145) (9.73418, 0.376394) (9.74779, 0.391819) (9.7614, 0.407589) (9.77502, 0.423565) (9.78863, 0.439609) (9.80224, 0.455585) (9.81585, 0.471367) (9.82947, 0.486835) (9.84308, 0.501881) (9.85669, 0.51641) (9.87031, 0.530343) (9.88392, 0.543614) (9.89753, 0.556176) (9.91115, 0.567997) (9.92476, 0.579062) (9.93837, 0.589371) (9.95198, 0.598939) (9.9656, 0.607795) (9.97921, 0.615979) (9.99282, 0.623542) (10.0064, 0.63054) (10.0201, 0.637039) (10.0337, 0.643106) (10.0473, 0.64881) (10.0609, 0.65422) (10.0745, 0.659403) (10.0881, 0.66442) (10.1017, 0.669327) (10.1153, 0.674173) (10.129, 0.678997) (10.1426, 0.683831) (10.1562, 0.688695) (10.1698, 0.693602) (10.1834, 0.698552) (10.197, 0.703537) (10.2106, 0.708543) (10.2242, 0.713545) (10.2379, 0.718515) (10.2515, 0.723419) (10.2651, 0.72822) (10.2787, 0.732878) (10.2923, 0.737355) (10.3059, 0.741613) (10.3195, 0.745614) (10.3332, 0.749325) (10.3468, 0.752717) (10.3604, 0.755763) (10.374, 0.758439) (10.3876, 0.760728) (10.4012, 0.762612) (10.4148, 0.764077) (10.4284, 0.765111) (10.4421, 0.765702) (10.4557, 0.765835) (10.4693, 0.765498) (10.4829, 0.764673) (10.4965, 0.76334) (10.5101, 0.761477) (10.5237, 0.759057) (10.5373, 0.75605) (10.551, 0.752421) (10.5646, 0.748134) (10.5782, 0.743152) (10.5918, 0.737435) (10.6054, 0.730944) (10.619, 0.723642) (10.6326, 0.715495) (10.6463, 0.706472) (10.6599, 0.696549) (10.6735, 0.685709) (10.6871, 0.673943) (10.7007, 0.661249) (10.7143, 0.647639) (10.7279, 0.633132) (10.7415, 0.617759) (10.7552, 0.60156) (10.7688, 0.584588) (10.7824, 0.566905) (10.796, 0.548582) (10.8096, 0.529698) (10.8232, 0.510339) (10.8368, 0.490598) (10.8504, 0.470572) (10.8641, 0.450359) (10.8777, 0.430061) (10.8913, 0.409777) (10.9049, 0.389604) (10.9185, 0.369637) (10.9321, 0.349965) (10.9457, 0.33067) (10.9594, 0.311827) (10.973, 0.293503) (10.9866, 0.275756) (11.0002, 0.258635) (11.0138, 0.242177) (11.0274, 0.226413) (11.041, 0.211361) (11.0546, 0.197034) (11.0683, 0.183435) (11.0819, 0.170557) (11.0955, 0.158391) (11.1091, 0.14692) (11.1227, 0.136122) (11.1363, 0.125972) (11.1499, 0.116443) (11.1635, 0.107504) (11.1772, 0.0991267) (11.1908, 0.0912792) (11.2044, 0.0839318) (11.218, 0.0770555)},
calib/range/.initial={8.37261:11.28},
calib/hist/.initial={(8.37261, 0.0633594) (8.78795, 0.0633594) (8.78795, 0.126719) (9.20329, 0.126719) (9.20329, 0.190078) (9.61863, 0.190078) (9.61863, 0.380156) (10.034, 0.380156) (10.034, 0.760313) (10.4493, 0.760313) (10.4493, 0.696954) (10.8647, 0.696954) (10.8647, 0.190078) (11.28, 0.190078)},
calib/kde/.initial={(8.37261, 0.0383196) (8.38722, 0.0385735) (8.40183, 0.0387733) (8.41644, 0.0389236) (8.43105, 0.0390303) (8.44566, 0.0391) (8.46027, 0.0391402) (8.47488, 0.0391592) (8.48949, 0.0391661) (8.5041, 0.0391705) (8.51871, 0.0391828) (8.53332, 0.0392139) (8.54793, 0.0392748) (8.56254, 0.0393771) (8.57715, 0.0395327) (8.59176, 0.0397532) (8.60637, 0.0400506) (8.62098, 0.0404366) (8.63559, 0.0409225) (8.6502, 0.0415195) (8.66481, 0.0422383) (8.67942, 0.0430888) (8.69403, 0.0440807) (8.70864, 0.0452227) (8.72325, 0.0465225) (8.73786, 0.0479874) (8.75247, 0.0496234) (8.76708, 0.0514355) (8.78169, 0.0534281) (8.7963, 0.055604) (8.81091, 0.0579654) (8.82552, 0.0605132) (8.84013, 0.0632475) (8.85474, 0.0661671) (8.86935, 0.0692701) (8.88396, 0.0725536) (8.89857, 0.0760137) (8.91318, 0.0796461) (8.92779, 0.0834454) (8.9424, 0.0874057) (8.95701, 0.0915206) (8.97162, 0.0957833) (8.98623, 0.100186) (9.00084, 0.104723) (9.01545, 0.109384) (9.03006, 0.114163) (9.04467, 0.119052) (9.05928, 0.124042) (9.07389, 0.129127) (9.0885, 0.134299) (9.10311, 0.139551) (9.11772, 0.144875) (9.13233, 0.150265) (9.14694, 0.155715) (9.16155, 0.161219) (9.17616, 0.16677) (9.19077, 0.172364) (9.20538, 0.177994) (9.21999, 0.183657) (9.2346, 0.189347) (9.24921, 0.19506) (9.26382, 0.200791) (9.27843, 0.206535) (9.29304, 0.212288) (9.30765, 0.218046) (9.32226, 0.223802) (9.33687, 0.229554) (9.35148, 0.235296) (9.36609, 0.241022) (9.3807, 0.246727) (9.39531, 0.252406) (9.40992, 0.258054) (9.42453, 0.263664) (9.43914, 0.269231) (9.45375, 0.274749) (9.46836, 0.280212) (9.48297, 0.285616) (9.49758, 0.290954) (9.51219, 0.296223) (9.5268, 0.301418) (9.54141, 0.306535) (9.55602, 0.311571) (9.57063, 0.316526) (9.58524, 0.321397) (9.59985, 0.326185) (9.61446, 0.330892) (9.62907, 0.335521) (9.64368, 0.340075) (9.65829, 0.344561) (9.6729, 0.348986) (9.68751, 0.353358) (9.70212, 0.357688) (9.71673, 0.361989) (9.73134, 0.366273) (9.74595, 0.370555) (9.76056, 0.374851) (9.77517, 0.37918) (9.78978, 0.383558) (9.80439, 0.388005) (9.819, 0.392541) (9.83361, 0.397186) (9.84822, 0.401961) (9.86283, 0.406884) (9.87744, 0.411977) (9.89205, 0.417257) (9.90666, 0.422744) (9.92127, 0.428454) (9.93588, 0.434401) (9.95049, 0.4406) (9.9651, 0.447061) (9.97971, 0.453793) (9.99432, 0.460802) (10.0089, 0.46809) (10.0235, 0.475659) (10.0381, 0.483504) (10.0528, 0.491619) (10.0674, 0.499993) (10.082, 0.508613) (10.0966, 0.51746) (10.1112, 0.526513) (10.1258, 0.535748) (10.1404, 0.545135) (10.155, 0.554643) (10.1696, 0.564237) (10.1842, 0.573878) (10.1989, 0.583526) (10.2135, 0.593137) (10.2281, 0.602666) (10.2427, 0.612064) (10.2573, 0.621284) (10.2719, 0.630276) (10.2865, 0.638988) (10.3011, 0.647371) (10.3157, 0.655373) (10.3303, 0.662944) (10.345, 0.670037) (10.3596, 0.676603) (10.3742, 0.682598) (10.3888, 0.687978) (10.4034, 0.692703) (10.418, 0.696735) (10.4326, 0.700042) (10.4472, 0.702592) (10.4618, 0.70436) (10.4764, 0.705323) (10.4911, 0.705463) (10.5057, 0.704768) (10.5203, 0.703227) (10.5349, 0.700836) (10.5495, 0.697597) (10.5641, 0.693513) (10.5787, 0.688593) (10.5933, 0.68285) (10.6079, 0.676303) (10.6226, 0.668973) (10.6372, 0.660884) (10.6518, 0.652066) (10.6664, 0.64255) (10.681, 0.632371) (10.6956, 0.621567) (10.7102, 0.610177) (10.7248, 0.598244) (10.7394, 0.585809) (10.754, 0.572919) (10.7686, 0.559618) (10.7833, 0.545953) (10.7979, 0.531971) (10.8125, 0.517719) (10.8271, 0.503243) (10.8417, 0.488588) (10.8563, 0.473801) (10.8709, 0.458925) (10.8855, 0.444003) (10.9001, 0.429076) (10.9147, 0.414184) (10.9294, 0.399366) (10.944, 0.384656) (10.9586, 0.370089) (10.9732, 0.355696) (10.9878, 0.341507) (11.0024, 0.327549) (11.017, 0.313845) (11.0316, 0.300419) (11.0462, 0.28729) (11.0608, 0.274475) (11.0755, 0.26199) (11.0901, 0.249847) (11.1047, 0.238057) (11.1193, 0.226628) (11.1339, 0.215565) (11.1485, 0.204874) (11.1631, 0.194557) (11.1777, 0.184614) (11.1923, 0.175045) (11.2069, 0.165846) (11.2216, 0.157014) (11.2362, 0.148544) (11.2508, 0.14043) (11.2654, 0.132664) (11.28, 0.12524)},
}
